Contrastive Learning of Features between Images and LiDAR

Image and Point Clouds provide different information for robots. Finding the correspondences between data from different sensors is crucial for various tasks such as localization, mapping, and navigation. Learning-based descriptors have been developed for single sensors; there is little work on cross-modal features. This work treats learning cross-modal features as a dense contrastive learning problem. We propose a Tuple-Circle loss function for cross-modality feature learning. Furthermore, to learn good features and not lose generality, we developed a variant of widely used PointNet++ architecture for point cloud and U-Net CNN architecture for images. Moreover, we conduct experiments on a real-world dataset to show the effectiveness of our loss function and network structure. We show that our models indeed learn information from both images as well as LiDAR by visualizing the features.

==> algorithms/algorithm1.tex <==
\begin{algorithm}[H]
    \caption{Range Image Preprocessing }
    \label{alg:algorithm1}
    \begin{algorithmic}
      \INPUT$I_{\text{mask}}$, $I_{\text{range}}$, $I_{\text{label}}$,$I_{\text{reflectivity}}$}.
      \STATE{$\hat{I}_{\text{mask}} = Closing(I_{\text{mask}})$}
      \STATE{$I_{\text{stripe}} = \hat{I}_{\text{mask}} - I_{\text{mask}}$}
      \STATE{$\hat{I}_{\text{range}} = NSInpainting(I_{\text{range}},I_{\text{stripe}})$}
      \STATE{$\hat{I}_{\text{reflectivity}} = NSInpainting(I_{\text{reflectivity}},I_{\text{stripe}})$}
      \STATE{$\hat{I}_{\text{label}} = NNInpainting(I_{\text{label}},I_{\text{stripe}})$}
    \end{algorithmic}
  \end{algorithm}

==> equations/all_loss.tex <==
\begin{equation}
    \label{eqn:all_loss}
        L = \lambda_PL_{P} + \lambda_BL_{B}
\end{equation}

==> equations/alpha.tex <==
\begin{equation}
\begin{aligned}
\alpha_{j}^{-}&=\gamma\max(s_j^-+m,0)\\
\alpha_{i}^{+}&=\gamma\max(1+m-s_i^+,0)\\ 
\end{aligned}
\label{alpha}
\end{equation}

==> equations/bigtriangleup.tex <==
\begin{equation}
\begin{aligned}
\bigtriangleup^{-}&=m\\
\bigtriangleup^{+}&=1-m\\ 
\end{aligned}
\label{bigtriangleup}
\end{equation}

==> equations/circle_loss.tex <==
{\small  
\begin{equation}
\mathcal{L} 
=\log \left[1+\sum_{j=1}^{L} \exp \left( \alpha_{j}^{-}\left(s_{j}^{-}-\bigtriangleup^{-}\right)\right) \sum_{i=1}^{K} \exp \left(\alpha_{i}^{+}\left(s_{i}^{+}-\bigtriangleup^{+}\right)\right)\right]
\label{circle_loss}
\end{equation}}

==> equations/earlystop_weightn.tex <==
{\small  
\begin{equation}
w_{j}^{-} = \max(1,\min(1-(s_{min}^{+}-s_{j}^{-})/r,0))
\end{equation}}

==> equations/earlystop_weightp.tex <==
\begin{equation}
w_{i}^{+} =
  \begin{cases}
    1-s_{i}^{+}   & \quad  s_{i}^{+}<0 \text{ or } s_{i}^{+}>s_{max}^{-}\\
    1   & \quad  otherwise\\
  \end{cases} 
\end{equation}

==> equations/feature_rep.tex <==
$x=\left(x_{pr},x_{sh}\right)$

==> equations/l_norm.tex <==
\begin{equation}
  \label{eqn:l_norm}
    L_{norm} = \frac{1}{N}\sum_{i=0}^N|\frac{e^{r_i}-e^{1/r_i}}{e^{r_i}+e^{1/r_i}}|
\end{equation}

==> equations/margin.tex <==
\begin{equation}
\begin{aligned}
m_{j}^{-}&=1-(1-s_{min}^{+})\times2\\
m_{i}^{+}&=0.0\\ 
\end{aligned}
\label{reunified_loss}
\end{equation}

==> equations/similarity.tex <==
\begin{equation}
\begin{aligned}
s^{+}&=f\left(x,x^{+}\right)\\
s^{-}&=f\left(x,x^{-}\right)\\
\end{aligned}
\end{equation}

==> equations/tuplecircle_sn.tex <==
{\small
\begin{equation}
\begin{aligned}
\mathcal{S}^{-}_{inertia} &=\sum_{j=1}^{N-1} \exp \left(\alpha_{img_j}^{-}\left(s_{img_j}^{-}-\bigtriangleup^{-}\right)\right)\\
                 &+\sum_{j=1}^{N-1} \exp \left(\alpha_{pcd_j}^{-}\left(s_{pcd_j}^{-}-\bigtriangleup^{+}\right)\right)\\
\mathcal{S}^{-}_{cross} &=\sum_{j=1}^{2N-1} \exp \left(\alpha_{j}^{-}\left(s_{j}^{-}-\bigtriangleup^{-}\right)\right)\\
\end{aligned}
\label{circle_loss}
\end{equation}}

==> equations/tuplecircle_sp.tex <==
{\small
\begin{equation}
\begin{aligned}
\mathcal{S}^{+}_{inertia} &= \exp \left( \alpha_{img}^{+}\left(s_{img}^{+}-\bigtriangleup^{+}\right)\right)\\
                  &+\exp \left( \alpha_{pcd}^{+}\left(s_{pcd}^{+}-\bigtriangleup^{+}\right)\right)\\
\mathcal{S}^{+}_{cross} &=\sum_{j=1}^{4} \exp \left( \alpha_{j}^{+}\left(s_{sh_j}^{+}-\bigtriangleup^{+}\right)\right)\\
\end{aligned}
\label{circle_loss}
\end{equation}}

==> equations/unified_loss.tex <==
{\small  
\begin{equation}
\begin{aligned}
\mathcal{L} &=\log \left[1+\sum_{i=1}^{K} \sum_{j=1}^{L} \exp \left(\gamma\left(s_{j}^{-}-s_{i}^{+}+m\right)\right)\right] \\
&=\log \left[1+\sum_{j=1}^{L} \exp \left(\gamma\left(s_{j}^{-}+m\right)\right) \sum_{i=1}^{K} \exp \left(\gamma\left(-s_{i}^{+}\right)\right)\right]
\end{aligned}
\label{unified_loss}
\end{equation}}

==> equations/weighted_unified_loss.tex <==
{\small 
\begin{equation}
\begin{aligned}
\mathcal{L}_{u n i} 
=\log\left[1+\sum_{j=1}^{L} \exp \left(\gamma w_{j}^{-}\left(s_{j}^{-}-m_{j}^{-}\right)\right) \sum_{i=1}^{K} \exp \left(-\gamma w_{i}^{+}\left(s_{i}^{+}-m_{i}^{+}\right)\right)\right]
\end{aligned}
\end{equation}
}

==> equations/weighted_unified_loss2.tex <==
\begin{equation}
\begin{aligned}
\mathcal{L} &=\log\left[1+SE^{-}\times SE^{+}\right]\\
SE^{-}&=\sum_{j=1}^{L} \exp \left(\gamma w_{j}^{-}\left(s_{j}^{-}-m_{j}^{-}\right)\right)\\
SE^{+}&=\sum_{i=1}^{K} \exp \left(-\gamma w_{i}^{+}\left(s_{i}^{+}-m_{i}^{+}\right)\right)\\ 
\end{aligned}
\label{reunified_loss}
\end{equation}

==> figures/img_viz.tex <==
\begin{figure}[h]
\begin{center} 
\begin{table} 
\begin{tabular}{c} 
\includegraphics[width=0.45\textwidth]{images/5_1/flabeled_img.png}\\(a) \\
\includegraphics[width=0.45\textwidth]{images/5_1/labeled_img.png}\\(b)\\
\end{tabular} 
\caption{Example} 
\label{fig:img_viz}
\end{table} 
\end{center} 
\end{figure}

==> figures/label_viz.tex <==
\begin{center} 
\begin{figure} 
\begin{tabular}{c} 
\includegraphics[width=0.45\textwidth]{images/5_1/flabeled_img.png}\\(a) \\
\includegraphics[width=0.45\textwidth]{images/5_1/labeled_img.png}\\(b)\\
\includegraphics[width=0.45\textwidth]{images/5_1/flabeled_pcd.png}\\(c) \\
\includegraphics[width=0.45\textwidth]{images/5_1/labeled_pcd.png}\\(d)\\
\includegraphics[width=0.45\textwidth]{images/5_1/kmean2d_img.png}\\(e)\\
\end{tabular} 
\caption{\textbf{Feature KMean Clustering Visualization}: (a) Full feature  clustering results of the full feature of image; (b) Shared feature clustering results of  image; (c) Full feature clustering results of  point cloud; (d) Shared feature clustering results of point cloud; (e) Pixel coordinate clustering results.} 
\label{fig:label_viz}
\end{figure} 
\end{center}  

==> figures/match_viz2.tex <==
\begin{figure}[h]
\includegraphics[width=0.45\textwidth]{images/8_1/mis_match.png}
\caption{\textbf{Cross-modality Matching Visualization}: Green and Blue circles represent points from the point cloud and image individually; Red lines denote the mismatching; (Note single green due to the small distance between two mismatched points.)} 
\label{fig:match_viz}
\end{figure}

==> figures/pcd_viz.tex <==
\begin{figure}[h]
  \centering
    \begin{tabular}{c}
    %\centering
     \includegraphics[width=0.45\textwidth]{images/5_1/flabeled_pcd.png} \\
     (a)\\
     \includegraphics[width=0.45\textwidth]{images/5_1/labeled_pcd.png} \\
      (b) \\
    \end{tabular}
    \caption{Hill Example (a) RGB Image, (b) Image Label, (c) Single Scan, (d) Multiple Scans}    
    \label{fig:img_viz}
\end{figure}
